PolarStar: Expanding the Scalability Horizon of Diameter-3 Networks

We present PolarStar, a novel family of diameter-3 network topologies derived from the star product of low-diameter factor graphs. PolarStar gives the largest known diameter-3 network topologies for almost all radixes, thus providing the best known scalable diameter-$3$ network. Compared to current state-of-the-art diameter-$3$ networks, PolarStar achieves $1.3\times$ geometric mean increase in scale over Bundlefly, $1.9\times$ over Dragonfly, and $6.7\times$ over {3-D} HyperX. PolarStar has many other desirable properties, including a modular layout, large bisection, high resilience to link failures and a large number of feasible configurations for every radix. We give a detailed evaluation with simulations of synthetic and real-world traffic patterns and show that PolarStar exhibits comparable or better performance than current diameter-3 networks.

==> allreduce_fig.tex <==
\begin{figure}[!htpb]
    \centering    \includegraphics[width=0.8\linewidth]{figures/Allreduce_SST_new.pdf}
    \caption{Performance of Allreduce Collective.}
\label{fig:sst_allreduce}
\end{figure}


==> conclusion.tex <==
\section{Conclusion}
We presented \newfly -- a novel diameter-3 network topology based on star product of factor graphs. 
\newfly exhibits state-of-the-art scalability
for diameter-3 networks with $1.9\times$ and $1.3\times$ geometric mean increase in scale over Dragonfly and state-of-the-art Bundlefly, \looseness=-1respectively.
We also develop a routing scheme for \newfly using its theoretical properties, and demonstrate comparable or better performance than existing diameter-3 networks for various synthetic and real-world motifs.
\newfly also has several desirable properties including a modular layout, a large design-space, high bisection bandwidth, and is amenable to bundling of global links into cost-effective multi-core fibers. 

==> diameter-3_new_proof.tex <==
\begin{propertyp}{R$^*$}\label{prop_R_star} A graph $G'$ 
satisfies Property~\ref{prop_R_star} if there is an involution $f$ on $G'$ so that for any $x'$ and $y' \in G'$, at least one of the following is true: 
\begin{enumerate}[itemsep=1pt,parsep=2pt]
    \item $y'=x'$
    \item $y'=f(x')$
    \item $y' \in f(N(x'))$
    \item $y' \in N(f(x'))$
\end{enumerate}
\end{propertyp}
\begin{theoremEnd}[end, restate, text link={See
\hyperref[proof:prAtEnd\pratendcountercurrent]{proof} in Section~\ref{sec:appendix} (the Appendix).}, text proof = {}, ]{proposition}
\label{proposition:Rstar}
A graph $G'$ of degree $d'$ having Property~\ref{prop_R_star} has at most $2d'+2$ vertices.
\end{theoremEnd}
\begin{proof}
    \begin{proofEnd}
   Fix some vertex $x'$ in $G'$. We will count how many other vertices there can be. Let $y'$ be any vertex in $G'$. By Property~\ref{prop_R_star}, at least one of the following is true:
	\begin{enumerate}[itemsep=1pt,parsep=2pt]
	\item $y' = x'$, giving exactly one choice for $y'$.
	\item $y'= f(x')$: Since $f$ is a bijection, then there is exactly one choice for $y'$.
	\item $y'\in f(N(x'))$: Since $N(x')$ has $\deg(x')$ vertices and $f$ is a bijection, there are exactly $\deg(x')$ choices for $y'$.
	\item $y'\in N(f(x'))$, giving exactly $\deg(f(x'))$ choices for for $y'$.
   \end{enumerate}
   Altogether, we have at most $2 + \deg(x') + \deg(f(x'))$ total vertices, assuming all conditions are disjoint. Since $\deg(x') \le d'$ and $\deg(f(x')) \le d'$, $G'$ can have at most $2+2d'$ vertices.
\end{proofEnd}
\end{proof}

\kledit{Lemma~\ref{lemma:2h_paths} states that any pair any pair of vertices in adjacent supernodes of the star graph $G_*$ are reachable within two hops from each other.
\begin{lemma}\label{lemma:2h_paths}
    Let $G_*=G*G'$ be a star product where $G'$ has Property~\ref{prop_R_star} and $G$ has Property~\ref{prop_R}. For any pair of adjacent vertices $x$ and $y$ in $G$, the shortest distance between any vertices $(x,x')$ and $(y,y')$ in $G_*$ is at most $2$.
\end{lemma}
\begin{proof}
    Since $x$ and $y$ are adjacent supernodes, $\left((x,x'),(y,f(x')\right)$ and $\left((x,f^(-1)(y')), (y,y')\right)$ are edges in $G_*$.
    From property~\ref{prop_R_star}, either of the following is true for any $x'$ and $y'$:
    \begin{enumerate}
        \item $y'=x' \rightarrow $ since $G$ has Property~\ref{prop_R}, 
        there exists a 2-hop path $(x,z,y)$ in $G$. Correspondingly, $\left((x,x'), (z,f(x')), (y,x'=y')\right)$ is a 2-hop path in $G_*$.
        \item $y'=f(x')\rightarrow$ $(y,f(x')=y')$ are adjacent in $G_*$.
        \item $y'\in f(N(x')) \rightarrow$ $x'$ and $f^{-1}(y')$ are adjacent in $G'$. Hence, $\left((x,x'), (x,f^(-1)(y')), (y,y')\right)$ is a 2-hop path in $G_*$.
        \item $y'\in N(f(x')) \rightarrow$ $\left((x,x'), (y,f(x')), (y,y')\right)$ is a 2-hop path in $G_*$.
    \end{enumerate}
    For any $x'$ and $y'$, there exists a path of length at most $2$ between $(x,x')$ and $(y,y')$ if $x$ and $y$ are adjacent in $G$, which proves the lemma.
\end{proof}
}

\begin{proof}
    Follows from the definition of the \lmedit{bijective} star product, and the fact that $f^2(x')=x'$ for all $x'$.
\end{proof}
\if0
\begin{proposition}\label{proposition:Rstar}
A graph $G'$ of degree $d'$ having Property~\ref{prop_R_star} has at most $2d'+2$ vertices.
\end{proposition}
\begin{proof}
   Fix some vertex $y$ in $G'$. We will count how many other vertices there can be. Let $x$ be a vertex in $G'$. By Property~\ref{prop_R_star}, at least one of the following is true:
	\begin{enumerate}[itemsep=1pt,parsep=2pt]
	\item $y = x$, giving exactly one choice for $x$.
	\item $y= f(x)$: Since $f$ is a bijection, then there is exactly one choice for $x$, namely $f^{-1}(y)$.
	\item $(x,y) \in E(G')$, giving $\deg(y)$ choices for $x$.
	\item $(f(X), f(y)) \in E(G')$: since $f$ is a function, $f(y)$ is fixed. Therefore there are $\deg(f(y))$ choices for $x$.
   \end{enumerate}
   Altogether, we have at most $2 + \deg(y) + \deg(f(y))$ total vertices, assuming all conditions are disjoint. Since $\deg(y) \le d'$ and $\deg(f(y)) \le d'$, $G'$ can have at most $2+2d'$ vertices.
\end{proof}
\fi
\if0
\vspace{-3mm}
\begin{theoremEnd}[end, restate, text link={See
\hyperref[proof:prAtEnd\pratendcountercurrent]{proof} in Section~\ref{sec:appendix} (the Appendix).}, text proof = {}]{corollary}
\label{corollary:Rstar}
A graph $G'$ satisfies Property~\ref{prop_R_star} if and only if for any $x'\in V(G')$, 
\begin{align}
V(G') &= \{x'\}\cup \{f(x')\} \cup f(N(x')) \cup N(f(x')) \nonumber \\
&= \{f(x')\}\cup \{x'\} \cup f(N(f(x'))) \cup N(x'). \nonumber
\end{align}
\end{theoremEnd}\begin{proof}
    \begin{proofEnd}
Consider the graph with edges $E(G')\cup f(E(G')) \cup \{(x',f(x')) | x'\in V(G')\}$.
The neighbors of a vertex $x'$ in this 
graph are given by $\{f(x')\}\cup N(x') \cup f(N(f(x'))$. By Property~\ref{prop_R_star}, this is a complete graph on $V(G')$.
Hence, 
$$
V(G')=\{x',f(x')\}\cup N(x') \cup f(N(f(x'))
$$
For each $x'\in V(G')$, $f(x')$ is also in $V(G')$.
Since $f$ is an involution on $V(G')$,
by substituting $y'=f(x')$ in the above, we get that for all $y'\in V(G')$,
\begin{equation}
\begin{aligned}
V(G')&=\{y',f(y')\}\cup N(f^{-1}(y')) \cup f(N(y')) \\\nonumber
\implies V(G')&=\{y',f(y')\}\cup N(f(y')) \cup f(N(y'))
\end{aligned}
\end{equation}

Clearly, the edges $E(G')\cup f(E(G')) \cup \{(x',f(x')) | x'\in V(G')\}$ give a complete graph over $V(G')$ iff $V(G')=\{x',f(x')\}\cup N(x') \cup f(N(f(x'))$, for all vertices $x'$.
\end{proofEnd}
\end{proof}
\fi
\if0
\begin{corollary}\label{corollary:Rstar}
A graph $G'$ satisfies Property~\ref{prop_R_star} if and only if for any $x'\in V(G')$, 
\begin{align}
V(G') &= \{x'\}\cup \{f(x')\} \cup f(N(x')) \cup N(f(x')) \nonumber \\
&= \{f(x')\}\cup \{x'\} \cup f(N(f(x'))) \cup N(x'). \nonumber
\end{align}
\end{corollary}
\begin{proof}
    See Corollary~\ref{appendix_corollary:Rstar} in Section~\ref{sec:appendix} (the Appendix).
\end{proof}
\fi
The following Property \ref{prop_R_1} is Property $P_i$ in \cite{bermond82} for the special case $i=1$, which is needed for diameter-$3$ star products.

\begin{propertyp}{R$_1$}\cite{bermond82}\label{prop_R_1}  A graph $G'$  has Property~\ref{prop_R_1} if there is a bijection $f$, with $f^2$ an automorphism of $G'$, so that the set of edges 
$
E(G') \cup f(E(G'))
$
is the entire set of edges in the complete graph on \looseness=-1$V(G')$.
\end{propertyp}












==> mb_table.tex <==
\begin{table}[ht] 
\centering
%\scriptsize
%\ssmall
%\sf
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccc@{}}
\toprule
%
\makecell{\textbf{Degree}\\ \textbf{(Radix)}} & 
\makecell{\textbf{Best known} \\ \textbf{Order}} 
 & \makecell{\textbf{Moore-bound}\\ \textbf{Efficiency}}
& \makecell{\textbf{\newfly}\\ \textbf{Order}} &
\makecell{\textbf{Moore-bound} \\ \textbf{Efficiency}} \\
%
\midrule
$18$ & $1,729^\ast$ & $31.3\%$ & $\mathbf{1,830}$ & $\mathbf{33.3\%}$\\
$19$ & $2,106^\dagger$ & $32.3\%$ & $\mathbf{2,128}$ & $\mathbf{32.6\%}$ \\
$20$ & $2,379^\ast$ & $31.2\%$ & $\mathbf{2,394}$ & $\mathbf{31.4\%}$\\
%
%
%
%
\bottomrule
\end{tabular}
}
%\vspaceSQ{-1em}
\caption{For radixes $18$-$20$, \newfly surpasses the previously largest known diameter-3 graphs. The previous results marked with an $*$ are from \cite{bermond82} and the one marked with a $\dagger$ is from \cite{bundlefly_2020}}%\vspace{-2mm}}
\label{tab:leaderboard}
\end{table} 

==> minpath_old.tex <==
\subsection{Minimal Path computation in PolarStar}\label{sec:minpath}
\kledit{
We use the properties of structure graph $G$ and supernode $G'$ to compute each minimal path (minpath) in PolarStar. The structure graph is an \emph{Erd\H os-R\'enyi} polarity graph with diameter $D=2$ and has Property~\ref{prop_R}.
We describe minpaths in Inductive-Quad supernode that satisfies Property~\ref{prop_R_star}; computation for Paley supernode is similar.

Let the source be $(z,z')$ and destination be $(y,y')$. 
If $(z,z')$ and $(y,y')$ are adjacent, minpath is just the edge $\left((z,z'),(y,y')\right)$. 
Next, we compute 2-hop minpaths when $z$ and $y$ are adjacent supernodes. These paths are graphically illustrated in Figure~\ref{fig:diameter_theorem} when routing from $(z,z')=(a_1,f(x'))$ to $(y,y')$ which is in an adjacent supernode.
We compute these paths by substituting $x'=f(z')$ in Property~\ref{prop_R_star}, which
gives the following exhaustive conditions:
\begin{enumerate}[label=(\alph*),itemsep=0pt,parsep=2pt]
    \item $y'=x'=f(z') \rightarrow$ $(y,y')$ and $(z,z')$ are adjacent.
    \item $y'=f(x')=z'\rightarrow$ From Property~\ref{prop_R}, there is a 2-hop path $(z,b,y)$ in structure graph $G$.
    Corresponding minpath in $G_*$ is $\left((z,z'), (b,f(z')), (y,z')\right)$ (Figure~\ref{fig:diameter_p1}). 
    \item $(y',x'=f(z'))\in E(G')\rightarrow$ minpath is $\left((z,z'), (y,f(z')), (y,y')\right)$ (Figure~\ref{fig:diameter_p2}).
    \item $(f(y'),f(x')=z')\in E(G')\rightarrow$ minpath is $\left((z,z'), (z,f(y')), (y,y')\right)$ (Figure~\ref{fig:diameter_p3}).
\end{enumerate}

Thus, we have a 2-hop minpath between all nodes in adjacent supernodes.
Lastly, we consider the case when $(z,z')$ and $(y,y')$ are neither adjacent nor in adjacent supernodes. From Property~\ref{prop_R}, there exists a 2-hop path $(z,a,y)$ in $G$. In $G_*$, we hop from $(z,z')$ to $(a,f(z'))$. 
Since $(a,f(z'))$ is in a supernode adjacent to $(y,y')$, we then take the 2-hop path to $(y,y')$ as described above, giving an overall path of length at most 3.
Paths between non-adjacent supernodes are shown in Figure~\ref{fig:diameter_theorem} with
source $(z,z')=(x,x')$.
}


==> sweep_3d_fig.tex <==
\begin{figure}[!htbp]
    \centering   \includegraphics[width=0.75\linewidth]{figures/Sweep3D.pdf}
    \caption{Performance of Sweep3D Motif. \lmcomment{Can we put Figs 11 and 12 as subfigures in the same figure?}}
    \label{fig:sst_sweep}
\end{figure}
